An Abstraction-Preserving Block Matrix Implementation in Maple

A Maple implementation of partitioned matrices is described. A recursive block data structure is used, with all operations preserving the block abstraction. These include constructor functions, ring operations such as addition and product, and inversion. The package is demonstrated by calculating the PLU factorization of a block matrix.

==> IfExistsUseBBL.tex <==
% arXiv doesn't run bibtex, so  we use \IfFileExists to test for *this* file to conditionalize \input of .bbl rather than using bibtex.
